Introducing Ensemble Machine Learning Algorithms for Automatic Test Case Generation using Learning Based Testing

Ensemble methods are powerful machine learning algorithms that combine multiple models to enhance prediction capabilities and reduce generalization errors. However, their potential to generate effective test cases for fault detection in a System Under Test (SUT) has not been extensively explored. This study aims to systematically investigate the combination of ensemble methods and base classifiers for model inference in a Learning Based Testing (LBT) algorithm to generate fault-detecting test cases for SUTs as a proof of concept. We conduct a series of experiments on functions, generating effective test cases using different ensemble methods and classifier combinations for model inference in our proposed LBT method. We then compare the test suites based on their mutation score. The results indicate that Boosting ensemble methods show overall better performance in generating effective test cases, and the proposed method is performing better than random generation. This analysis helps determine the appropriate ensemble methods for various types of functions. By incorporating ensemble methods into the LBT, this research contributes to the understanding of how to leverage ensemble methods for effective test case generation.

==> sec_conclusion.tex <==
This study explores the effectiveness of using ensemble methods for model inference in LBT. We conduct experiments with nine different ensemble combinations for two software under test (SUT) scenarios involving classification and numeric functions. 
We assess the effectiveness of the generated test cases using each ensemble method and compare their mutation scores for the two SUTs against the performance of the test suite created by random generation. The results indicate that Boosting ensemble techniques outperform Bagging methods on average regarding mutation score. This observation aligns with the incremental learning technique of Boosting methods, likely contributing to their better performance. This insight is valuable for software testing practitioners, guiding the selection of appropriate ensemble methods for model inference in test case generation.

%Overall, this work broadens the horizon of software testing by incorporating ensemble learning techniques and highlights the potential benefits of using Boosting methods in test case generation. 
Overall, this research serves as a stepping stone for future investigations into optimizing test case generation methods, advancing the state-of-the-art in software testing, and improving the reliability and robustness of software systems.
%In our future work we will try to use more ensemble combinations to check effectiveness of test suites generated by those ensemble methods. As we have already discussed in the previous section that we only implemented a limited number of combinations for the model inference. Implementing LBT with vast number of ensemble combinations and checking mutation testing for various SUTs may provide us more concrete result about effectiveness of any specific ensemble combination. More over as the test case generation was random, we would like to implemented different test generation technique like category partition and check any improvement from the random method. Oracle generation method like Metamorphic testing can also be integrated in LBT for test case generation. As already discussed before, mutation testing is not a complete evaluation for adequacy of the test suite. We need to check the adequacy of the test cases in terms of coverage as well. Comparing our approach with other LBT methods is another important experiment to find out how much effective test cases are being generated through the proposed ensemble based LBT method. 
% In the future, we plan to explore a wider range of ensemble combinations to assess their effectiveness in generating test suites. 
% By incorporating a vast number of ensemble combinations and testing them on various SUTs, we aim to obtain more robust and conclusive results regarding the effectiveness of specific ensemble combinations.
% Furthermore, we will explore different test generation techniques, such as category partitioning, to compare their performance with the random method used in this study. 
% To gain further insights into the efficiency of our proposed ensemble-based LBT method, we will compare it with other existing LBT approaches. 
% This comparative analysis will help us determine how effectively our approach generates test cases compared to alternative methods.

==> sec_data_availability.tex <==
The data and artifacts of this paper are available for access at the following link: \textcolor{blue}{\href{https://figshare.com/s/9ef8ee16f157864b4802}{https://figshare.com/s/9ef8ee16f157864b4802}}. 
%Currently, the program committee has the privilege to access it through the provided link. 
% However, upon acceptance of the paper, we intend to make it publicly available to all interested individuals.

==> sec_related_work.tex <==
%Several implementations of Learning-Based Testing (LBT) have been developed as a proof of concept.
\textbf{\textit{LBT}.} There are two important parts of LBT, which are model inference using the test cases and generation and selection of inputs.
Each of the following implementations demonstrates different approaches to leveraging LBT for various aspects of software testing by bringing variations in these two parts. 

In the case of model inference, some notable examples include: 1) The Model-Inference driven Testing (MINTEST) framework proposed by Papadopoulos and Walkinshaw~\cite{papadopoulos2015black}, the BESTEST approach by Fraser and Walkinshaw~\cite{fraser2015assessing}, MELBA by Briand et al.~\cite{briand2009using} utilized the C4.5 Decision Tree learner for model inference, 2) Fraser and Walkinshaw~\cite{walkinshaw2017uncertainty} employed the Genetic Programming Inference Engine for model inference~\cite{o2009riccardo} to generate the models, 3) Ghani and Clark~\cite{ghani2008strengthening} proposed the use of a reverse-engineered Daikon model for inference by identifying test cases that differ from the model, 4) Meinke and Sindhu \cite{meinke2011incremental}, LearnLib by Raffelt et al.~\cite{raffelt2005learnlib} used state machines for model inference, 5) Meinke and Niu~\cite{meinke2010learning} used n-dimensional polynomial models for model inference.

%State machine has also been used for the model inference step. Meinke and Sindhu \cite{meinke2011incremental} , LearnLib by Raffelt et al. cite{raffelt2005learnlib} uses state machines for model inference. Meinke and Niu \cite{meinke2010learning} used n-dimensional polynomial models for model inference.
For input generation, the process can be random~\cite{papadopoulos2015black}, or they can be based on coverage of input~\cite{fraser2015assessing}. 
Category-Partition technique has also been used for this purpose~\cite{briand2009using}. 

%Though LBT has been been mostly used for procedural programs, approach to test reactive systems using LBT has also been proposed \cite{meinke2011incremental}. A reactive system is a software system such as robotic machines, flights controls that interacts continuously with its environment over time \cite{meinke2011learning}. 
%This technique has been used to generate test cases for both systems with discrete and numeric output~\cite{fraser2015assessing}.

While LBT has primarily found application in procedural programs, there have been proposals to extend its usage to test reactive systems as well~\cite{meinke2011incremental}. 
Reactive systems refer to software systems, such as robotic machines or flight controls, continuously interacting with their environment over time~\cite{meinke2011learning}.
By leveraging LBT, testing methodologies for reactive systems can be enhanced, allowing for efficient and effective validation of their dynamic behavior and interactions. 
Meinke and Sindhu~\cite{meinke2013lbtest} introduced LBTest, a pragmatic tool designed for testing reactive systems utilizing LBT. Subsequently, Feng et al.~\cite{feng2013case} effectively employed LBTest to identify bugs in three distinct industrial systems, and remarkably, the tool successfully detected bugs in each of these systems.
Notably, this technique has also been successfully employed to generate test cases for both systems with discrete and numeric output~\cite{fraser2015assessing}.

\textbf{\textit{Ensemble Method.}} Ensemble methods have also been applied for test cases and Oracle generation. Hershkovich et al.~\cite{hershkovich2021prioritized} employed Gradient Boosting as a means to prioritize test case generation for a specific and limited section of the software component. 
%Their objective was to minimize the efforts required for test execution. By utilizing this approach, they aimed to focus resources on the most critical areas of the software, thereby optimizing the testing process and ensuring more efficient use of resources. 
Braga et al.~\cite{braga2018machine} utilized the AdaBoostM1 ensemble method to generate test oracles for the ``Shopping Cart" web application, designed for purchase management. 
Arrieta et al.~\cite{arrieta2021using} and Gartziandia et al.~\cite{gartziandia2022machine} employed an ensemble method in conjunction with various other ML algorithms to generate test oracle for elevators dispatching algorithms, with the ensemble method demonstrating superior performance. 
%Among all the algorithms utilized, the ensemble method demonstrated superior performance, outperforming the other approaches. 
Utting et al.~\cite{utting2020identifying} employed Gradient Boosting to detect areas with inadequate test coverage in a Bus Tracking system and a Supply Chain Management software.
%, analyzing log files from customer reports to identify weakly-tested portions.
%to detect areas with inadequate test coverage in a Bus Tracking system and a Supply Chain Management software. They achieved this by analyzing the log files obtained from customer reports, allowing them to pinpoint the weakly-tested portions of the systems more effectively.
Eidenbenz et al.~\cite{eidenbenz2021boosting} utilized an AdaBoostedTree algorithm to forecast inputs that may lead to failures in a power grid control system, facilitating the identification of problem-causing inputs and improving failure prevention.
%to automatically forecast inputs that may lead to failures in a power grid control system. By leveraging this approach, they aimed to identify potential problem-causing inputs more efficiently, enabling better anticipation and prevention of failures within the power grid control system avoiding the simulation approach which is expensive. Ensemble method has aslo been used to source code driven fault prediction in program as well.

%Kumar et al.~\cite{kumar2017using} used Majority Voting Ensemble to predict faults in open-source projects using source code metrics. Yang et al.~\cite{yang2017tlel} used a Two-layer ensemble learning method to detect 70\%  bugs of large open-source projects using only 20\% of the source code.


%Ensemble methods have proven to be particularly noteworthy in the context of fault prediction within space technology-based systems. This is especially crucial because, in space missions, software systems must operate flawlessly 100\% of the time. Twala~\cite{twala2011predicting} used ensemble methods to create a fault prediction system using datasets from  NASA metrics data program (MDP) data repository. Saifudin et al.~\cite{saifudin2019tackling} utilized an ensemble approach to address the issue of class imbalance in NASA's datasets for fault prediction. The class imbalance problem is crucial to tackle because software defects represent a minority class in the data. If the dataset is not balanced, the prediction results often favor the majority class, leading to the potential oversight of many defects.

%Ensemble methods have found application in numerous other fields for fault prediction in software systems, and research has consistently demonstrated their superiority over individual classifiers in software defect prediction~\cite{mabayoje2018software,laradji2015software}. 
% Ensemble methods have been successful in fault prediction for open-source projects based on source code metrics. Kumar et al.~\cite{kumar2017using} utilized Majority Voting Ensemble, while Yang et al.~\cite{yang2017tlel} employed a Two-layer ensemble learning method, achieving the detection of 70% of bugs in large open-source projects using only 20% of the source code.
% Additionally, ensemble methods have shown significant promise in the context of fault prediction within space technology-based systems. Twala~\cite{twala2011predicting} used ensemble methods with datasets from NASA metrics data program (MDP) data repository for fault prediction. Saifudin et al.~\cite{saifudin2019tackling} applied an ensemble approach to address class imbalance in NASA's datasets, which is crucial due to software defects being a minority class in the data. 
% Moreover, ensemble methods have been widely applied in various fields for fault prediction in software systems, consistently demonstrating their superiority over individual classifiers in software defect prediction~\cite{mabayoje2018software, laradji2015software}.


==> sec_threats.tex <==
%\subsection{Threats to external validity}
%The answers to RQ1 and RQ2 can only be validly applied to the functions for which we have generated test cases and conducted mutation testing. We have only used two SUTs where one is a classification function another is a numeric function. As our experiment was only a proof of concept for using ensemble methods for LBT, It is possible that the answers for the research questions could change if conduct experiment on vast set of SUTs.

%Apart from that, we have used a limited set of ensemble combinations for our experiment. There are other supervised algorithms which could have been used for both AdaBoost and Bagging algorithms. Another threat is that for the base estimators DecisionTree, LogisticRegression we have used the default parameters from scikit-learn library. We have used only 100 base estimators for each combinations. Parameters for the ensemble methods Bagging and AdaBoost was default values as well.  Variations of those parameters in a combination could provide different result.

%Parameters for the random input generator is another threat. The choice for the parameters for the random input generation for both the SUTs has a fixed range. Changing this range could have generated different set of test cases for which mutation score could be different.

%We have generated a limited number of test cases using each combination of ensemble for this experiment. More variation in test cases would change the number of mutants killed for a test suite.

%The set of utility function chosen for both of the SUT can impact the result. For example, Almulla and Gay \cite{almulla2020learning} used reinforcement learning to adaptively search the fitness function that can select test cases which has higher possibility for triggering exception in program.

%In addition, we have only conducted mutation testing to compare the effectiveness of the generated test suites. Mutation testing only provides a quantitative adequacy measures of a specific test set, and not numeric or probabilistic results about coverage as such and does not provide any feedback on how to improve an inadequate test set~\cite{meinke2004automated}.

\textbf{External Validity.} The applicability of the answers to Research Questions RQ1 and RQ2 is limited to the functions for which we generated test cases and conducted mutation testing. 
Our experimentation involves only two SUTs: one being a classification function and the other a numeric function. 
While our SUTs are widely used representative programs, our experiment primarily serves as a proof of concept for using ensemble methods in LBT. 
Therefore, it is essential to acknowledge that the answers to the research questions may vary when applied to a broader set of SUTs.

\textbf{Internal Validity.} The limited set of ensemble combinations used in our experiment poses a potential threat. Other supervised algorithms could have been considered for both AdaBoost and Bagging algorithms. Moreover, for the base estimators DecisionTree and LogisticRegression, we use default parameters from the scikit-learn library. The use of different parameter configurations in a combination might lead to different outcomes.

%Additionally, the default parameter values for the ensemble methods Bagging and AdaBoost could be considered as another potential limitation. Modifying these parameter values could yield varied results.
%The parameters selected for the random input generator also pose a threat. The fixed range for the random input generation in both SUTs could have resulted in a different set of test cases, influencing the mutation score.
%It is important to acknowledge that the limited number of test cases generated for each ensemble combination in this experiment might not fully capture the variation required to comprehensively assess the impact on the number of mutants killed in a test suite. Conducting experiments with a more extensive range of test cases could provide further insights.

\textbf{Conclusion Validity.} The mutation score we have calculated relies on the process of creating mutants by seeding the original program. In our experiment, we solely utilized $\mu$BERT for generating the mutants. 
It is crucial to acknowledge that if mutants were created using other mutation techniques, the quality of mutations might vary significantly, potentially leading to drastic changes in our results. 
Therefore, the choice of mutation technique can have a substantial impact on the accuracy and validity of the mutation score, and it is an important factor to consider when interpreting the results of our study.

\textbf{Construct Validity.} We exclusively utilize mutation testing to compare the effectiveness of the generated test suites. 
While mutation testing offers quantitative adequacy measures for a specific test set, it does not yield numeric or probabilistic results concerning coverage. 
Moreover, mutation testing does not provide feedback on how to enhance an inadequate test set~\cite{meinke2004automated}.
Therefore, it is crucial to consider alternative evaluation methods or additional techniques to gain a more comprehensive understanding of the test suite's quality and potential areas for improvement.

%\subsection{Threats to internal validity}
%The mutation score that we have calculated depend on how the mutants are created by seeding the original program. In our experiment, we have only used $\mu$BERT to create the mutants. If the mutants were created using other mutation framework, the quality of the mutants could differ and that can cause drastic change in our results.



%We had to analyze full papers when necessary to mitigate this bias.
